Hypergraph burning, matchings, and zero forcing

Lazy burning is a recently introduced variation of burning where only one set of vertices is chosen to burn in the first round. In hypergraphs, lazy burning spreads when all but one vertex in a hyperedge is burned. The lazy burning number is the minimum number of initially burned vertices that eventually burns all vertices. We give several equivalent characterizations of lazy burning on hypergraphs using matchings and zero forcing, and then apply these to give new bounds and complexity results. We prove that the lazy burning number of a hypergraph $H$ equals its order minus the maximum cardinality of a certain matching on its incidence graph. Using this characterization, we give a formula for the lazy burning number of a dual hypergraph and give new bounds on the lazy burning number based on various hypergraph parameters. We show that the lazy burning number of a hypergraph may be characterized by a maximal subhypergraph that results from iteratively deleting vertices in singleton hyperedges. We prove that lazy burning on a hypergraph is equivalent to zero forcing on its incidence graph and show an equivalence between skew zero forcing on a graph and lazy burning on its neighborhood hypergraph. As a result, we show that finding an upper bound on the lazy burning number of a hypergraph is NP-complete, which resolves a conjecture from \cite{BJR}. By applying lazy burning, we show that computing an upper bound on the skew zero forcing number for bipartite graphs is NP-complete. We finish with open problems.

==> caleb-core-alg.tex <==

Given a hypergraph $H$ and $L\subseteq V(H)$, the {\em weak induced subhypergraph} is the hypergraph $H\setminus L$ with vertex set $V(H)\setminus L$ and the edge set consists of $e\setminus L$ for $e\in E(H)$ and $e\not\subseteq L$. 
% That is, $H\setminus L$ has edge set $\{ e\cap (V(H)\setminus L) : e\in E(H), e\cap (V(H)\setminus L)\neq \emptyset\}$.


\begin{algorithm}[H]
\label{core_H}

\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{a hypergraph $H=(V,E)$}

\Output{the core of $H$, $C_H$}

\BlankLine

initialize $C_H=H$

\Repeat{$C_H$ is unchanged}{%contains no singleton edges}{

\ForAll{$e\in E(C_H)$}{

\If{$|e|=1$}{

Delete both $e$ and the vertex it contains from $C_H$

}

}

}

\Return{$C_H$}
\text{(the core of $H$)}

\caption{Construct the core of $H$.}
\end{algorithm}

\begin{lemma}
Algorithm \ref{core_H} runs in time at most $\mathcal{O}(nm^2),$ where $|V(H)|=n$ and $|E(H)|=m$.
\end{lemma}

\begin{proof}
Each iteration of the outer loop (lines 2-8) deletes at least one vertex from $C_H$ except for the last iteration. Hence, the outer loop executes at most $n+1$ times. Each instance of the inner loop (lines 3-7) iterates over at most $m$ objects. The operation in line 4 takes constant time. Finally, consider the operation in line 5. Denote the unique vertex in $e$ by $v$. Deleting $v$ from $V(C_H)$ and $e$ from $E(C_H)$ takes constant time. However, the algorithm must also delete $v$ from each other edge in $H$ that contained it, which accounts for at most $m$ more operations.
\end{proof}

Perhaps unsurprisingly, we can characterize lazy burning sets using the concept of cores. This is interesting because $C_H$ is a rigorously defined set-theoretic object that is independent of the rules of the lazy hypergraph burning game.

\begin{theorem}
\label{core_equals_lazy_burning}
If $H$ is a hypergraph and $L\subseteq V(H)$, then $L$ is a lazy burning set for $H$ if and only if the core of $H\setminus L$ is empty.
\end{theorem}

\begin{proof}
For the forward implication, assume $L$ is a lazy burning set for $H$ and let $u_1,\ldots,u_k$ be an ordering of $V(H)\setminus L$ such that the earlier a vertex burns in the lazy burning process, the earlier it appears in the list (with ties broken arbitrarily). We will prove that none of the vertices $u_i$ are in the core of $H\setminus L$ by induction on $i$.

For the base case, $u_1$ burns in the first propagation step because it belongs to some edge $e$ that contains no other unburned vertices. If $e$ was a singleton edge, then $u_1$ gets deleted and hence does not belong to $C_{H\setminus L}$. Otherwise, each other vertex in $e$ belongs to $L$, and hence the corresponding edge in $H\setminus L$ contains only $u_1$. Hence, $u_1$ gets deleted in this case as well.

Now, assume each of $u_1,u_2,\ldots,u_i$ gets deleted while constructing $C_{H\setminus L}$. Consider the edge $e$ that causes $u_{i+1}$ to burn in the lazy burning game. By the definition of our ordering, no vertex in $e$ is of the form $u_j$ with $j>i+1$. Now, consider the corresponding edge in $H\setminus L$. It contains only vertices from the set $\{ u_1,u_2,\ldots,u_{i+1} \}$ (that is, no vertices from $L$ or with a higher index than $i+1$). Since each of $u_1,\ldots,u_i$ gets deleted while constructing $C_{H\setminus L}$, $e$ eventually contains only the vertex $u_{i+1}$, so $u_{i+1}$ gets deleted.

For the reverse implication, assume the core of $H\setminus L$ is empty and let $u_1,\ldots,u_k$ be an ordering of $V(H)\setminus L$ such that the earlier a vertex gets deleted (via Algorithm \ref{core_H}), the earlier it appears in the list (with ties broken arbitrarily). We will prove that each of the vertices $u_i$ burn in $H$ when $L$ is burned as a lazy burning set by induction on $i$.

For the base case, since $u_1$ was deleted from $H\setminus L$ in the first step of the algorithm, it must belong to some singleton edge $e$ in $H\setminus L$. Consider the corresponding edge in $H$. If it is still a singleton (that is, it contains no vertices from $L$), then $u_1$ burns via spontaneous combustion. Otherwise, the corresponding edge in $H$ only contains $u_1$ as well as vertices from $L$, so $u_1$ burns via propagation.

Now, assume each of $u_1,u_2,\ldots,u_i$ is burned. Consider the edge $e$ that contains $u_{i+1}$ and causes it to be deleted from $H\setminus L$ (via Algorithm \ref{core_H}). Denote the corresponding edge in $H$ by $e^\prime$. If $e^\prime$ is also a singleton, then $u_{i+1}$ burns via spontaneous combustion. Otherwise, $e^\prime$ becomes the singleton edge $e$ (containing only $u_{i+1}$) after deleting $L$ and a series of vertex deletions via the algorithm. Suppose $e^\prime$ contains vertices of the form $u_j$ with $j>i+1$. For this edge to become a singleton containing only  $u_{i+1}$, $u_j$ must be deleted strictly before $u_{i+1}$, which contradicts our ordering of $V(H)\setminus L$. Hence, $e^\prime$ is an edge in $H$ that contains only vertices from the set $L\cup\{ u_1,\ldots, u_{i+1}\}$. Observe that $u_{i+1}\in e^\prime$. Since each of $u_1,\ldots,u_i$ eventually burns, at some point in the lazy burning process $e^\prime$ contains only burned vertices and $u_{i+1}$, and hence $e^\prime$ causes $u_{i+1}$ to burn via propagation. 
\end{proof}


% \begin{comment}
\begin{theorem}

    For any hypergraph $H$, $b_L(H)=b_L(C_H)$.
\end{theorem}

\begin{proof}
    We first show that every optimal lazy burning set for $H$ is a subset of $C_H$. In particular, we do this by showing that all of $H\setminus C_H$ burns when $L=\emptyset$ is chosen as the lazy burning set. Let $v_1,v_2,\ldots,v_k$ be an ordering of the vertices of $H\setminus C_H$ such that the earlier a vertex is deleted from $H$ via Algorithm \ref{core_H}, the earlier it appears in the list. For the base case, $v_1$ was deleted first since it belonged to a singleton edge in $H$, so $v_1$ burns in $H$. Now, assume $v_1,v_2,\ldots, v_{i-1}$ are all burned in $H$. Consider the edge $e$ that caused $v_i$ to be deleted during the execution of Algorithm \ref{core_H}. If $e$ was a singleton in $H$ (before any deletions), then  $v_i$ will burn. Otherwise, $e$ became a singleton after a series of deletions. But the only vertices that could have been deleted from $e$ before it became a singleton are those in $\{v_1,v_2,\ldots,v_{i-1}\}$. Hence, in $H$ (before any deletions), $e\subseteq \{v_1,\ldots,v_i\}$. Since $v_i$ is the only unburned vertex in this edge, it burns.

    Next, we prove $b_L(H)\leq b_L(C_H)$. Let $L$ be an optimal lazy burning set for $C_H$, and let $u_1,\ldots,u_k$ be an ordering of the vertices of $C_H\setminus L$ such that the earlier a vertex burns in $C_H$, the earlier it appears in the list (with ties ordered arbitrarily). We will show that $L$ is a lazy burning set for $H$ by induction. For the base case, consider the edge $e$ that causes $u_1$ to burn in $C_H$. Note that $e\subseteq L\cup\{u_1\}$. Now, if the corresponding edge in $H$ contains no additional vertices, then $u_1$ burns in $H$ immediately. Otherwise, the corresponding edge in $H$ contains vertices from $L\cup\{u_1\}$ as well as those from $H\setminus C_H$. But every vertex in $H\setminus C_H$ will eventually burn, so $u_1$ will eventually be the unique unburned vertex in this edge, and hence, it will burn. Now, assume $u_1,u_2,\ldots,u_{i-1}$ are all burned in $H$. Consider the edge $e$ that caused $u_i$ to burn in $C_H$. Apart from $u_i$, it can only contain vertices from $L\cup\{u_1,u_2,\ldots,u_{i-1}\}$. Hence, apart from $u_i$, the corresponding edge in $H$ contains only vertices from $L$, $\{u_1,u_2,\ldots,u_{i-1}\}$, and/or $H\setminus C_H$, all of which are eventually burn. Therefore, this edge causes $u_i$ to burn in $H$.

    Finally, we prove $b_L(H)\geq b_L(C_H)$. Let $L$ be an optimal lazy burning set for $H$, so $L\subseteq C_H$. Let $u_1,u_2,\ldots,u_k$ be an ordering of the vertices of $C_H\setminus L$ such that the earlier a vertex burns in $H$, the earlier it appears in the list (with ties ordered arbitrarily). The order in which the vertices of $H\setminus C_H$ burn is not relevant. Note that $u_i\in C_H$ for each $i$, and hence no edge in $H$ containing $u_i$ is a singleton. We will show that $L$ is a lazy burning set for $C_H$ by induction. For the base case, consider the edge $e$ that causes $u_1$ to burn in $H$. Apart from $u_1$, the only vertices that can belong to $e$ are those from $L$ and $H\setminus C_H$. Hence, the corresponding edge in $C_H$ is a subset of $L\cup\{u_1\}$, so $u_1$  in $C_H$. Now, assume $u_1,u_2,\ldots,u_{i-1}$ are all burned in $C_H$. Consider the edge $e$ that caused $u_i$ to burn in $H$. Apart from $u_i$, it can only contain vertices from $L$, $H\setminus C_H$, and/or $\{u_1,u_2,\ldots,u_{i-1}\}$. Hence, the corresponding edge in $C_H$ contains only vertices from $L$ and $\{u_1,u_2,\ldots,u_i\}$, all of which are burned except for $u_i$, so this edge causes $u_i$ to burn.
    \end{proof}

\begin{corollary}
    $L$ is a lazy burning set for $H$ if and only if $L\cap C_H$ is a lazy burning set for $C_H$.
\end{corollary}
% \end{comment}

\textcolor{blue}{Use above corollary (whose proof is very similar to the above thm) in complexity result!}

Note that the lazy burning number of $C_H$ is the same regardless of whether or not spontaneous combustion is allowed, as $C_H$ contains no singletons. 






\begin{corollary}
\label{no_SC_NP_comp}
    Let $H$ be a hypergraph. The decision problem \emph{``Is $b_L(H)\leq k$?''} is NP-complete when spontaneous combustion is not allowed.
\end{corollary}

\begin{proof}
    Consider an arbitrary hypergraph $H$. If $H$ has no singleton edges, then this decision problem is equivalent to the one from Theorem~\ref{SC_NP_complete}, so assume $H$ has singleton edges. We will show that a solution to the original model of lazy burning yields a solution to lazy burning with spontaneous combustion on $H$, and hence, the original model is ``at least as hard.'' The proof will follow, as the original model of lazy burning is known to be in NP \cite{burgess2024extendinggraphburninghypergraphs}.

    Given $H$, we first compute $C_H$, which notably only takes polynomial time. Let $L$ be an optimal lazy burning set for $C_H$ in the original model. We then note that $L$ is also an optimal lazy burning set for $C_H$ when spontaneous combustion is allowed. Finally, by Theorem~\ref{core_bl_equality} and its proof, $L$ is an optimal lazy burning set for $H$ when spontaneous combustion is allowed.
\end{proof}

\textcolor{blue}{Caleb: is the above proof formal enough? Maybe use the following proof instead:
Suppose we wish to answer the question ``is $b_L(H)\leq k$?'' (with spontaneous combustion), and we have the answer to the question ``is $b_L(C_H)\leq k$?'' (without spontaneous combustion). If $b_L(C_H)\leq k$, then $b_L(H)\leq k$ (with spontaneous combustion) since any lazy burning set for $C_H$ is a lazy burning set for $H$ (see the proof of Theorem~\ref{core_bl_equality}). Otherwise, $b_L(C_H)> k$ (without spontaneous combustion). Suppose $b_L(H)\leq k$ (with spontaneous combustion). There exists a lazy burning set $L$ for $H$ of size at most $k$. By the same argument as the proof of Theorem~\ref{core_bl_equality}, $L\cap C_H$ is a lazy burning set for $C_H$ (without spontaneous combustion). Since $|L\cap C_H|\leq |L|\leq k$, we have that $b_L(C_H)\leq k$ (without spontaneous combustion), which is a contradiction. Thus, $b_L(H)> k$ (with spontaneous combustion), so a solution to ``is $b_L(C_H)\leq k$?'' yields a solution to the NP-complete decision problem from Theorem~\ref{SC_NP_complete}.
Therefore, original lazy burning is NP-complete on the family of hypergraphs that are the cores of other hypergraphs. Since it is in NP \cite{burgess2024extendinggraphburninghypergraphs}, it is NP-complete in general.
}


% ------- 



\begin{theorem}\label{zero_set_equivalence}
If $H$ is a hypergraph and $L\subseteq V(H)$, then $L$ is a lazy burning set for $H$ if and only if $L\cup E(H)$ is a zero forcing set for $\mathrm{IG}(H)$.
\end{theorem}

\begin{proof}
For the forward implication, assume $L$ is a lazy burning set for $H$ and let $u_1,u_2,\ldots,u_k$ be an ordering of $V(H)\setminus L$ such that the earlier a vertex burns in the lazy burning process, the earlier it appears in the list (with ties broken arbitrarily). We claim that $L\cup E(H)$ is a zero forcing set in $\mathrm{IG}(H)$. In particular, we will prove that the vertices corresponding to $u_1,u_2,\ldots,u_k$ in $\mathrm{IG}(H)$ will become forced using induction on $i$. This will prove the claim, seeing as these are the only unforced vertices in $\mathrm{IG}(H)$ at the start of the game.

For the base case, $u_1$ burns in the first propagation step because it belongs to some edge $e$ that contains no other unburned vertices. Hence, in $\mathrm{IG}(H)$, $e$ is a forced vertex whose only unforced neighbor is $u_1$, so $e$ forces $u_1$.

Now assume each of $u_1,u_2,\ldots,u_i$ becomes forced in $\mathrm{IG}(H)$. Consider the edge $e$ that causes $u_{i+1}$ to burn in the lazy burning game. By the definition of our ordering, no vertex in $e$ is of the form $u_j$ with $j>i+1$. Hence, in $\mathrm{IG}(H)$, $e$ is a forced vertex whose open neighborhood is a subset of $\{ u_1,u_2,\ldots,u_{i+1}\}$ (and $eu_{i+1}\in E(\mathrm{IG}(H))$ is guaranteed). Since $u_{i+1}$ is unforced and each of $u_1,u_2,\ldots,u_i$ is forced, $u_{i+1}$ is the unique unforced neighbor of $e$. Hence, $e$ forces $u_{i+1}$.
 
For the reverse implication, assume $L\cup E(H)$ is a zero forcing set for $\mathrm{IG}(H)$. Let $u_1,\ldots,u_k$ be an ordering of $V(H)\setminus L$ such that the earlier a vertex becomes forced, the earlier it appears in the list (with ties broken arbitrarily). We will prove that each of the vertices $u_i$ burns in $H$ when $L$ is burned as a lazy burning set by induction on $i$.

For the base case, since $u_1$ becomes forced in the first time step, it must be the unique unforced neighbor of some vertex $e$, where $e$ belongs to the partite set of vertices that is indexed by $E(H)$. Consider the edge in $H$ corresponding to $e$ (and call it $e$ also for simplicity). We have that $u_1\in e$ in $H$. In $\mathrm{IG}(H)$, each neighbor of $e$ belongs to the zero forcing set except for $u_1$. Thus, in $H$, each vertex in $e$ belongs to the lazy burning set except for $u_1$, so $u_1$ burns via propagation.

Now assume each of $u_1,u_2,\ldots,u_i$ is burned in $H$. Consider the vertex $e$ in $\mathrm{IG}(H)$ that forces $u_{i+1}$. Since $e$ is adjacent to $u_{i+1}$, $e$ must belong to the partite set in $\mathrm{IG}(H)$ whose vertices are indexed by $E(H)$. Also, each other neighbor of $e$ must be forced in a time step strictly earlier than $u_{i+1}$, so the open neighborhood of $e$ in $\mathrm{IG}(H)$ is a subset of $\{ u_1,u_2,\ldots,u_{i+1}\}$. Hence, in $H$, $e$ is an edge that is a subset of $\{ u_1,u_2,\ldots,u_{i+1}\}$. Since $u_{i+1}$ is the only unburned vertex in this set and $u_{i+1}\in e$, $u_{i+1}$ burns due to propagation within $e$.
\end{proof}





\begin{theorem}
\label{inf_fam_tight_1}
    There exists an infinite family of hypergraphs for which the bound in Corollary~\ref{another_zero_bound} is tight.
\end{theorem}

\begin{proof}
    Consider the family of generalized stars constructed as follows. Given $k,\ell\geq 2$, define $H_{k,\ell}$ as the hypergraph with $\ell$ edges, each of which contains $k$ vertices of degree one, such that all edges intersect in a central vertex. More formally, $E(H_{k,\ell})=\{e_1,e_2,\ldots,e_\ell\}$ and $V(H_{k,\ell})=\{v,u_1^1,\ldots,u_k^1,\ldots,u_1^\ell,\ldots,u_k^\ell\}$ where $e_i=\{v,u_1^i,\ldots,u_k^i\}$ for each $i$. Note that $H_{k,\ell}$ is $(k+1)$-uniform.

    First, we show that $b_L(H_{k,\ell})=(k-1)\ell+1$. Any lazy burning set for $H_{k,\ell}$ must contain at least $k-1$ vertices of degree one in each edge. If any edge $e$ contains fewer than $k-1$ burned degree-one vertices at the start of the game, then that edge contains two or more unburned vertices of degree one. These vertices will never burn because $e$ will never contain exactly one unburned vertex. Hence, $b_L(H_{k,\ell})\geq(k-1)\ell$. However, if we choose $k-1$ degree-one vertices in each edge as their lazy burning set, then every edge will contain an unburned vertex of degree one, as well as $v$, which is also unburned, so no burning will spread. Hence, $b_L(H_{k,\ell})>(k-1)\ell$. Indeed, if we initially burn $k-1$ degree-one vertices per edge as well as $v$ then $H_{k,\ell}$ will burn in one round, so $b_L(H_{k,\ell})\leq(k-1)\ell+1$. 

    Since any optimal lazy burning set for $H_{k,\ell}$ contains a degree-one vertex in each edge, the maximum number of non-adjacent vertices one can choose from an optimal lazy burning set is $|E(H_{k,\ell})|=\ell.$ Hence, for this family of hypergraphs, the upper bound from Corollary~\ref{another_zero_bound} is $$b_L(H_{k,\ell})+|E(H_{k,\ell})|-x=b_L(H_{k,\ell})+\ell-\ell=b_L(H_{k,\ell}).$$
    
    We now consider the corresponding incidence graph $I_{H_{k,\ell}}$. Observe that $I_{H_{k,\ell}}$ may be viewed as a rooted tree, with $v$ as the root. The vertices $e_1$ through $e_\ell$ are all incident to $v$ and in the second layer of the tree, and the vertices $u_i^j$ are in the third layer of the tree (and they are all leaves). Now that $e_j$ is adjacent to each vertex $u_1^j,u_2^j,\ldots,u_k^j$. We will prove that $z(I_{H_{k,\ell}})=(k-1)\ell+1$, and the proof will be complete.

    First, for each vertex $e_j$, at least $k-1$ of the $k$ leaves incident to it must be initially forced. Otherwise, there are two or more unforced leaves incident to $e_j$, and hence $e_j$ will never have a unique unforced neighbor. Thus, the unforced leaves incident to $e_j$ will never become forced, so $z(I_{H_{k,\ell}})\geq (k-1)\ell$. Indeed, if we force exactly $k-1$ leaves per vertex $e_j$ (and force no other vertices), then the vertices $e_j$ will all immediately become forced. However, no more forcing will occur, as each vertex $e_j$ will be incident to two unforced vertices; $v$ and a leaf. Thus, $z(I_{H_{k,\ell}})> (k-1)\ell$. Indeed, if one forces $k-1$ leaves per vertex $e_j$ as well as $v$, then $I_{H_{k,\ell}}$ will become completely forced in two steps, so $z(I_{H_{k,\ell}})\leq (k-1)\ell+1$ and the proof is complete. 
\end{proof}



\begin{proof}
Let $L$ be an optimal lazy burning set for $H$, and let $S$ be the corresponding zero forcing set of size $b_L(H)+|E(H)|$ for $\mathrm{IG}(H)$. Denote the chosen vertices in $L$ by $v_1,v_2,\ldots,v_x$ and let $e_1,e_2,\ldots,e_x$ be a list of edges in $H$ such that $v_i\in e_i$ for each $i$. Observe that the neighborhoods of the vertices $v_i$ in $\mathrm{IG}(H)$ are disjoint. Hence, in $\mathrm{IG}(H)$, the vertices $v_i$ and $e_i$ are adjacent, and if $i\neq j$, then the vertices $v_i$ and $e_j$ are not adjacent. We claim that $S\setminus\{e_1,e_2,\ldots,e_k\}$ is a zero forcing set in $\mathrm{IG}(H)$. Each $v_i$ is part of the initially forced set, and $e_i$ is the only neighbor of $v_i$ that has been removed from the forcing set. As every neighbor of $v_i$ in $\mathrm{IG}(H)$ is forced except for $e_i$, $v_i$ will immediately force $e_i$. The proof follows, as $S$ is a forcing set for $\mathrm{IG}(H)$.
\end{proof}

